DRFLOW: A Deep Research Benchmark for Personalized Workflow Prediction

Deep research (DR) systems are increasingly used for complex information-seeking tasks, but existing works mainly focus on generating reports and summaries. In contrast, many enterprise tasks instead require an agent to identify concrete workflows which is a sequence of action-steps. For example, rather than summarizing budgeting policies, an agent should be able to determine the steps needed to answer a question such as: "How do I request new headcount given a fixed budget?". Therefore, we introduce DRFLOW, a benchmark for evaluating personalized workflows predicted by agents from heterogeneous sources. Each task requires the agent to identify relevant evidence from scattered sources, then use that evidence to predict the correct action-step sequence for the user's task. DRFLOW contains 100 tasks across five domains, with 1,246 reference workflow steps grounded in more than 3,900 sources. We define seven diagnostic metrics covering factual grounding, step recovery, structural ordering, condition resolution, and personalization. We further present DRFLOW-Agent (DRFA), a workflow-oriented reference agent to predict personalized workflow. We show that although DRFA improves over strong baseline agents (upto 10.02% average F1 score), there is substantial room for improvement remains across these workflow metrics, indicating that predicting complete and correct personalized workflows remains a challenging frontier for deep research.

==> Prompts/introductory_email_setup_part_1.tex <==
You are an expert in enterprise communication systems. Your task is to generate a realistic setup of users for an email thread.

Company: {company_name} - {company_description}
Industry: {industry}

Known Participants:
1. Company Representative:
   - Name: {persona_name}
   - Role: {persona_role}
   - Email: {persona_email}
   - Description: {persona_role_description}

2. External User/Client:
   - Name: {user_name}
   - Role: {user_role}
   - Email: {user_email}
   - Description: {user_role_description}

==> Prompts/introductory_email_setup_part_2.tex <==
Requirements:
- Generate 1-2 additional realistic business users (colleagues, managers, or partners) to make the thread feel authentic.
- Return ONLY a JSON array of users.
- The array MUST include the two known participants provided above, followed by the additional ones you generate.
- Use this structure for each user:
[
    {{
        "type": "user",
        "username": "firstname.lastname",
        "first_name": "Firstname",
        "last_name": "Lastname",
        "email": "firstname.lastname@company.com"
    }}
]

IMPORTANT:
- Do NOT include any preamble or extra text.
- Ensure the email addresses for additional users are realistic for the company or industry.

==> Prompts/introductory_email_thread_part_1.tex <==
You are an expert business communicator. Your task is to generate a realistic email thread of {num_messages} messages.

Company: {company_name} - {company_description}
Deep Research (DR) Question: {dr_question}

Email Setup (Participants):
{email_setup}

High-Level Sequence of Steps (to be subtly communicated):
{tasks_sequence}

Requirements:
1. Create a professional email thread where the participants discuss matters related to the company's business.
2. Start saying something like 'while you are completing the required steps, please note that...' from the persona {persona_name} sending an email to the user {user_name}. Do not mention any other information of the user or the persona.
3. The primary goal is to SUBTLY communicate the very high-level and brief sequence of some of the steps listed above to the user ({user_name}) for the purpose of the Deep Research (DR) Question: {dr_question}.
4. Do not add any new information or hallucinate any information outside the given step sequence.
5. Do not mention anything like 'First','Start with' etc. Becuase the user will think that the sequence is starting from here.
6. The conversation should feel natural, not like a direct list of instructions. It could be a project hand-off, a planning session, or a status update.

==> Prompts/introductory_email_thread_part_2.tex <==
7. The persona ({persona_name}) should be a key participant.
8. The thread must be {num_messages} messages long.
9. You must maintain the order of the tasks as listed above.
10. While describing the sequence, do not say 'simultaneously do that'. Because this will make the tasks look parallel, not sequential.
11. Remember to mention the tasks in high-level, brief, and subtle way, without revealing too much. Make the user work for the answer.


Output Format:
Return ONLY a JSON array with the following structure:
[
    {{
        "type": "email",
        "id": "email_001",
        "subject": "Realistic Subject Line",
        "from": "sender@company.com",
        "from_name": "Sender Name",
        "to": ["recipient@company.com"],
        "date": "2025-10-24 09:00:00",
        "body": "Email content..."
    }}
]

IMPORTANT:
- Return ONLY the JSON object, nothing else.
- The insight (sequence of steps) must be naturally embedded. Do not make the emails lengthy, detailed or repetitive.

==> Prompts/workflow_prompt_part_1.tex <==
You are an expert enterprise workflow architect. Generate a COMPREHENSIVE workflow report with **10-15** detailed, granular steps.

DR Question: "{context.original_question}"
User situation and persona: Infer from the DR question and from the retrieved documents (emails, chats, internal files) below.

### AVAILABLE SOURCES (use these IDs for citations):
{doc_ids_block}

### DOCUMENT CONTENTS:
{findings_text}

### SOURCE REFERENCE:
{sources_reference}

### CITATION FORMAT:
Use `[DOC:src_N]` format where src_N is a source ID from the list above (e.g., [DOC:src_1], [DOC:src_3]).
Cite policy documents for workflow rules and personal documents for user-specific facts.

**FACTUALITY REQUIREMENT**: In the Generic Workflow Steps and Personalized Workflow Steps (Section 1 and 2), cite ONLY src_N IDs that correspond to **internal sources** (policy documents, local files, emails, internal documents). Do NOT cite IDs that correspond to web or external search results in workflow step content.

---

# Research Report: Personalized Workflow Analysis

## Executive Summary
Summarize the workflow analysis citing key policy and personal evidence sources [DOC:src_N].

## 1. Generic Enterprise Workflow

### Overview
Extract a COMPREHENSIVE workflow from the policy documents. You MUST include EVERY distinct procedural step - aim for **10-15 detailed steps** covering the COMPLETE process from start to finish. Each step should represent a SINGLE discrete action (e.g., "Complete intake form" is one step, "Run gate check" is another, "Configure settings" is another). Do NOT merge multiple actions into one step.

### Generic Workflow Steps
```json
[
  {{
    "item": 1,
    "title": "Step title (e.g., 'Create X record', 'Complete intake form XYZ', 'Run gate check')",
    "task": "Brief task (e.g., 'Create a new onboarding workspace and attach handoff notes') [DOC:src_N]",
    "task_description": "DETAILED description (3-5 sentences) explaining exactly what to do, what specific fields to fill, what systems/tools/forms to use, what data to capture. Include ALL necessary details: form names or codes, system/tool names, specific fields, required attachments, who needs to be involved. [DOC:src_N]",
    "subtask_description": "For ANY step that has a decision/branch/conditional in the policy (if X then A, else B): you MUST put the FULL condition text HERE with ALL branches explicitly listed (e.g., 'If X -> select Y; else select Z.'). For steps with no branch, use empty string.",
    "prerequisite": "Item number of prerequisite step (e.g., '1') or empty string if this is the first step or has no dependency",
    "prerequisite_description": "Why the prerequisite must be completed first (e.g., 'The workspace record must exist before the intake form can be submitted')"
  }},
  {{
    "item": 2,
    "title": "Next step title",
    ...
  }}
  // Continue for ALL steps (aim for 10-15 total)
]
```

### GENERIC WORKFLOW REQUIREMENTS (CRITICAL):
- Extract EVERY distinct step from ALL policy documents - do NOT combine or skip steps
- Each step should be a SINGLE discrete action (creating a record, filling a form, running a check, configuring a setting, scheduling meeting, etc.)
- Include the FULL end-to-end process relevant to the DR question
- Keep descriptions DETAILED with specific form names, system names, field names, tool names mentioned in the policies
- CRITICAL: For EVERY step that involves a decision or branch or conditional (if/then/else, tier-based, count-based, type-based), you MUST fill subtask_description with the COMPLETE condition text listing ALL branches. Do NOT leave subtask_description empty for conditional steps.
- Look for conditions triggered by: tier/level selection, user counts/thresholds, feature or integration requirements, package types, approval status, validation outcomes
- Include prerequisites that show step dependencies (which step must complete before this one)
- **TARGET: 10-15 steps** (minimum 10 unless policy truly has fewer discrete actions; maximum 15).

### Generic Flowchart
```mermaid
graph TD
  A[Step 1] --> B[Step 2]
  B --> C{{Decision Point}}
  C -->|Condition X| D[Path X]
  C -->|Condition Y| E[Path Y]
  D --> F[Continue...]
```

==> Prompts/workflow_prompt_part_2.tex <==
## 2. Personalized Recommended Workflow

### User Situation Analysis
Extract key facts from user's personal evidence [DOC:src_N]:
- Specific entities mentioned (vendors, systems, people)
- Dates and timeframes
- Data types involved
- Constraints or special circumstances

**IMPORTANT**: Carefully search through ALL documents (especially emails, chats, and user-provided files) to extract user-specific facts. Look for:

**Source Types to Search:**
- **enterprise_email**: User's emails about the incident, vendor communications
- **enterprise_chat**: Mattermost/Slack/Teams messages about the situation
- **internal documents**: User's local files with specific details
- **persona block**: User role, responsibilities, constraints

**Facts to Extract** [DOC:src_N]:
- Specific entities: vendor names, system names, people involved
- Dates and timeframes: discovery date, incident timing, deadlines
- Data details: types of data, encryption status, affected counts
- Access facts: confirmed/denied access, subcontractor involvement
- Constraints: operational limits, survey windows, downtime restrictions
- User role: who they are, what they can approve

**List ALL facts found in documents:**
(Be explicit - list each fact found and cite the source document)

### Condition Resolution Table
For EACH step in the Generic Workflow that has a non-empty subtask_description, create ONE row below. Use the EXACT condition text from that step. Search ALL user evidence documents to determine which branch applies.

| Generic Condition (from subtask_description above) | User Evidence Found | Resolution |
|----------------------------------------------------|---------------------|------------|
| [Copy EXACT condition from step N's subtask_description] | [Specific user fact with DOC:src_N] or "No evidence found" | Resolved: [specific path chosen] OR Unresolved: keep condition |

**RESOLUTION RULES:**
- Search ALL available documents (emails, chats, user files) for evidence that determines which branch applies
- If user evidence clearly indicates which branch: mark "Resolved: [path]" and cite the evidence
- If no evidence found or evidence is ambiguous: mark "Unresolved: keep condition"
- You MUST have one row per conditional step - do not skip any

### Personalized Workflow Steps
**MANDATORY CITATIONS**: Every step MUST include [DOC:src_N] in task, task_description, AND justification. Use policy source IDs for process steps and personal source IDs (emails, user files) for user-specific facts. No step may be left without citations.

```json
[
  {{
    "item": 1,
    "title": "Personalized step title with user-specific details",
    "task": "PERSONALIZED task incorporating specific user facts - use actual names, numbers, systems from user evidence [DOC:src_N]",
    "task_description": "DETAILED personalized description using user's SPECIFIC facts. Replace generic terms with actual: names, system/tool names, counts, timeframes, tier or package names, deadlines, constraints from the evidence. Cite both policy and personal evidence. [DOC:src_N][DOC:src_M]",
    "subtask_description": "EMPTY string ('') if the Condition Resolution Table shows this condition as Resolved. KEEP the full conditional text if Unresolved.",
    "prerequisite": "Item number or empty",
    "prerequisite_description": "Same as generic or personalized if relevant",
    "justification": "Explain WHY this exact step is included in the personalized workflow for this user. State what policy requirement, user fact, or resolved condition makes the step necessary now; MUST end with [DOC:src_N] citations (policy and/or personal evidence)."
  }}
  // SAME NUMBER of steps as generic workflow. EVERY step: task, task_description, and justification MUST contain [DOC:src_N].
]
```

==> Prompts/workflow_prompt_part_3.tex <==
### PERSONALIZATION RULES:
1. **SAME NUMBER OF STEPS** as generic workflow
2. **PERSONALIZE task/task_description** with user's specific facts (dates, names, numbers, entities)
3. **Conditional branches**: If a condition in the generic workflow is RESOLVED by user's personal evidence, present the personalized workflow accordingly: use the single resolved path in the step title/task and leave subtask_description EMPTY. If the condition is NOT resolved by evidence, keep the conditional text in subtask_description so the user sees both branches.
4. **subtask_description**:
   - EMPTY ("") when user evidence resolves which path to take (condition is Resolved in table)
   - KEEP conditional text when evidence does NOT determine the path (condition is Unresolved)
5. **justification**:
   - Explain why this step belongs in the personalized workflow, not just what to do
   - Reference user's SPECIFIC facts that determine the applicable path
   - If the step is unconditional, explain what policy or user circumstance still makes it necessary
   - MUST cite both policy and personal evidence using [DOC:src_N]

### CITATION REQUIREMENTS FOR PERSONALIZED SECTIONS (MANDATORY):
- **Personalized Workflow Steps JSON**: Each of task, task_description, and justification MUST contain at least one [DOC:src_N]. Use valid source IDs from the AVAILABLE SOURCES list.
- **Section 3 (Step-by-Step Personalized Guidance)**: Each step's **Description** MUST end with [DOC:src_N]. At least one **Action Item** per step MUST cite a source, e.g. "[ ] Action detail [DOC:src_N]".


### EXAMPLE TRANSFORMATIONS:

**Generic step with condition (example):**
- task: "Select the appropriate option based on tier and size"
- subtask_description: "If tier is premium -> select option A; else select option B. If count exceeds threshold -> add additional pack; else keep default."

**Personalized (condition RESOLVED):**
- task: "Select option A and add the additional pack [DOC:src_1]"
- subtask_description: "" (empty because evidence resolved both conditions)
- justification: "Evidence shows premium tier and count above threshold [DOC:src_5], which triggers option A and the additional pack [DOC:src_1]."

**Personalized (condition NOT RESOLVED):**
- task: "Select option based on package type; determine which applies [DOC:src_1]"
- subtask_description: "If package is standard -> path X. If premium -> path Y."
- justification: "No evidence found specifying package type, so both branches must be preserved [DOC:src_1]."

### Personalized Flowchart
```mermaid
graph TD
  A[Personalized Step 1] --> B[Personalized Step 2]
  B --> C[Step 3]
  C --> D{{Unresolved Decision if any}}
```
Show resolved paths as direct arrows. Keep decision diamonds only for UNRESOLVED conditions.

## 3. Step-by-Step Personalized Guidance

For each step, provide. **You MUST add [DOC:src_N] citations** to every Description and to at least one Action Item per step (use valid source IDs from AVAILABLE SOURCES).

### Step N: [Title]
**Description**: Detailed personalized guidance. End with citation(s), e.g. "...per portal requirements [DOC:src_1]."
**Action Items**:
- [ ] Specific action with details [DOC:src_N]
- [ ] Additional actions as needed (cite where relevant)

## References
(Leave blank - auto-generated)

---

CRITICAL REQUIREMENTS:
1. Generate **10-15 DETAILED steps** in generic workflow - extract EVERY distinct procedural step from policy documents. If you have fewer than 10, you are merging steps; if you have more than 15, consolidate only where actions are truly atomic together.
2. For each step that has an if/then/else or decision or conditional in the policy, you MUST put that COMPLETE condition text in subtask_description with ALL branches listed
3. Condition Resolution Table: one row per conditional step, search ALL user evidence to resolve conditions
4. Personalized workflow has IDENTICAL number of steps as generic (10-15)
5. Personalize task/task_description with USER'S SPECIFIC FACTS (actual names, counts, systems, dates, constraints from evidence)
6. subtask_description in personalized: EMPTY when resolved by user evidence, KEEP condition text when NOT resolved
7. Every justification must reference specific user facts with citations
8. **CITATIONS (MANDATORY)**: Use [DOC:src_N] format. In the PERSONALIZED WORKFLOW (Section 2): every step's task, task_description, and justification MUST contain at least one [DOC:src_N]. In Section 3 (Step-by-Step Guidance): every step's Description and at least one Action Item per step MUST contain [DOC:src_N]. Only use source IDs from the AVAILABLE SOURCES list (src_1, src_2, etc.).

==> analyses.tex <==


%\input{analysis_qualitative}

==> prev_result_adv_bar_chart.tex <==
\paragraph{Performance of DRFA on Adversarial Split.}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figures/original_vs_adversarial_by_model.pdf}
    \caption{Comparison of DRFA on the original and adversarial splits across four backbone models. The X-axis shows backbone models, colors denote evaluation metrics, and hatched bars indicate the adversarial split.}
    \label{fig:adv_results}
\end{figure*}

Given DRFA's better performance on the original split, we further stress test it on an adversarial split designed to perturb grounding and workflow construction. Figure~\ref{fig:adv_results} shows a consistent degradation on the main structural and personalization axes across all four backbones. Averaged over models, F1 drops from $54.84$ to $50.74$, Condition Resolution drops from $38.21$ to $37.86$, and Personalized Comprehensiveness drops from $56.54$ to $51.57$.
%while Precision also declines from $46.14$ to $43.19$ and Recall from $68.30$ to $67.28$. Factuality, however, remains stable on average and slightly increases from $87.85$ to $89.02$.
Among the four backbones, Claude-Opus-4.5 is the most robust overall, with the smallest F1 decline;% unchanged Precision, and only modest reductions in Condition Resolution and Personalized Comprehensiveness; 
GPT-5.2 is also comparatively stable, whereas Gemini-3.1-pro-preview and especially DeepSeek-v3.2 exhibit larger degradations on the core end-to-end metrics. \textit{This consistent compression across core workflow metrics underscores the scope of improvement in robust personalized workflow synthesis.}

==> prev_table_adv_result.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4.2pt}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{llccccccc}
\toprule
\textbf{Model} & \textbf{Agent} & \textbf{Factuality} & \textbf{Recall} & \textbf{Precision} & \textbf{F1} & \textbf{Topology} & \textbf{Cond.~Res.} & \textbf{Pers.~Comp.} \\
\midrule
GPT-5.2 & DRBA & $86.41$\,\dn{3.60} & $58.13$\,\dn{2.30} & $37.30$\,\dn{14.81} & $44.36$\,\dn{9.81} & $86.52$\,\dn{3.11} & $24.58$\,\dn{0.27} & $42.61$\,\dn{2.38} \\
        & DRFA & $\mathbf{94.38}$\,\up{8.39} & $\mathbf{65.86}$\,\dn{3.57} & $\mathbf{47.96}$\,\dn{14.38} & $\mathbf{53.67}$\,\dn{10.23} & $\mathbf{90.04}$\,\dn{2.18} & $\mathbf{41.36}$\,\dn{1.47} & $\mathbf{55.67}$\,\dn{3.59} \\
\midrule
Claude-Opus-4.5 & DRBA & $\mathbf{86.78}$\,\up{1.42} & $63.70$\,\dn{1.49} & $37.86$\,\dn{6.90} & $44.52$\,\dn{6.57} & $\mathbf{93.10}$\,\up{4.63} & $23.59$\,\dn{2.40} & $39.56$\,\dn{2.33} \\
                & DRFA & $82.54$\,\dn{0.77} & $\mathbf{68.35}$\,\dn{3.72} & $\mathbf{47.43}$\,\dn{8.44} & $\mathbf{53.19}$\,\dn{7.51} & $89.68$\,\up{1.55} & $\mathbf{46.72}$\,\dn{0.46} & $\mathbf{58.51}$\,\dn{3.99} \\
\midrule
Gemini-3.1-pro & DRBA & $\mathbf{79.10}$\,\dn{11.14} & $47.75$\,\dn{8.19} & $\mathbf{24.24}$\,\dn{12.83} & $30.18$\,\dn{10.81} & $\mathbf{86.00}$\,\up{2.88} & $12.92$\,\dn{1.98} & $33.54$\,\up{3.16} \\
               & DRFA & $72.36$\,\dn{14.80} & $\mathbf{49.26}$\,\dn{18.05} & $24.07$\,\dn{18.48} & $\mathbf{30.42}$\,\dn{18.81} & $85.32$\,\dn{5.88} & $\mathbf{18.86}$\,\dn{8.12} & $\mathbf{42.32}$\,\dn{5.76} \\
\midrule
DeepSeek-v3.2 & DRBA & $81.32$\,\dn{12.25} & $48.55$\,\dn{11.93} & $30.36$\,\dn{8.53} & $34.04$\,\dn{11.33} & $\mathbf{83.13}$\,\dn{6.30} & $16.12$\,\up{1.10} & $27.26$\,\dn{6.25} \\
              & DRFA & $\mathbf{82.30}$\,\dn{12.62} & $\mathbf{51.35}$\,\dn{17.05} & $\mathbf{32.32}$\,\dn{16.13} & $\mathbf{38.34}$\,\dn{16.76} & $82.03$\,\dn{9.71} & $\mathbf{28.03}$\,\dn{7.82} & $\mathbf{51.83}$\,\dn{4.49} \\
\midrule
Average & DRBA & $\mathbf{83.40}$\,\dn{6.40} & $54.53$\,\dn{5.98} & $32.44$\,\dn{10.77} & $38.27$\,\dn{9.63} & $\mathbf{87.19}$\,\dn{0.47} & $19.30$\,\dn{0.89} & $35.74$\,\dn{1.95} \\
        & DRFA & $82.89$\,\dn{4.95} & $\mathbf{58.70}$\,\dn{10.60} & $\mathbf{37.95}$\,\dn{14.37} & $\mathbf{43.91}$\,\dn{13.32} & $86.77$\,\dn{4.05} & $\mathbf{33.74}$\,\dn{4.47} & $\mathbf{52.08}$\,\dn{4.46} \\
\bottomrule
\end{tabular}
}
\caption{Results on the mixed split of DRFA. Subscripts (in color) denote the absolute change relative to the original split (Table~\ref{tab:main_results}).}
\label{tab:adv_results}
\end{table*}



% \begin{table*}[!t]
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \resizebox{0.7\textwidth}{!}{
% \begin{tabular}{llccccccc}
% \toprule
% \textbf{Backbone} & \textbf{Agent} & \textbf{Factuality} & \textbf{Recall} & \textbf{Precision} & \textbf{F1} & \textbf{Topology} & \textbf{Cond.~Res.} & \textbf{Pers.~Comp.} \\
% \midrule
% GPT-5.2 & DRBA   & $88.14$\,\dn{1.87}  & $59.92$\,\dn{0.51}  & $50.76$\,\dn{1.35}  & $53.17$\,\dn{1.00}  & $83.97$\,\dn{5.66}  & $23.27$\,\dn{1.58}  & $42.61$\,\dn{2.38} \\
%         & DRFA & $84.29$\,\dn{1.70}  & $66.57$\,\dn{2.86}  & $61.20$\,\dn{1.14}  & $63.71$\,\dn{0.19}  & $91.49$\,\dn{0.73}  & $42.55$\,\dn{0.28}  & $55.67$\,\dn{3.59} \\
% \midrule
% Claude-Opus-4.5 & DRBA   & $86.78$\,\up{1.42}  & $63.70$\,\dn{1.49}  & $42.87$\,\dn{1.89}  & $39.52$\,\dn{11.57} & $93.10$\,\up{4.63}  & $23.59$\,\dn{2.40}  & $39.56$\,\dn{2.33} \\
%                 & DRFA & $82.54$\,\dn{0.77}  & $70.35$\,\dn{1.72}  & $47.43$\,\dn{8.44}  & $47.19$\,\dn{13.51} & $88.68$\,\up{0.55}  & $46.72$\,\dn{0.46}  & $58.51$\,\dn{3.99} \\
% \midrule
% Gemini-3.1-pro & DRBA   & $73.88$\,\dn{16.36} & $52.18$\,\dn{3.76}  & $35.68$\,\dn{1.39}  & $38.84$\,\dn{2.15}  & $83.38$\,\up{0.26}  & $14.57$\,\dn{0.33}  & $33.54$\,\up{3.16} \\
%                & DRFA & $85.89$\,\dn{1.27}  & $54.44$\,\dn{12.87} & $47.43$\,\up{4.88}  & $47.86$\,\dn{1.37}  & $90.00$\,\dn{1.20}  & $26.37$\,\dn{0.61}  & $42.32$\,\dn{5.76} \\
% \midrule
% DeepSeek-v3.2 & DRBA   & $80.79$\,\dn{12.78} & $54.58$\,\dn{5.90}  & $38.28$\,\dn{0.61}  & $48.82$\,\up{3.45}  & $88.22$\,\dn{1.21}  & $15.81$\,\up{0.79}  & $27.26$\,\dn{6.25} \\
%               & DRFA & $82.65$\,\dn{12.27} & $59.23$\,\dn{9.17}  & $44.83$\,\dn{3.62}  & $51.09$\,\dn{4.01}  & $90.39$\,\dn{1.35}  & $32.87$\,\dn{2.98}  & $51.83$\,\dn{4.49} \\
% \midrule
% Average & DRBA   & $82.40$\,\dn{7.40} & $57.59$\,\dn{2.92} & $41.90$\,\dn{1.31} & $45.09$\,\dn{2.82} & $87.17$\,\dn{0.50} & $19.31$\,\dn{0.88} & $35.74$\,\dn{1.95} \\
%         & DRFA & $\mathbf{83.84}$\,\dn{4.00} & $\mathbf{62.65}$\,\dn{6.66} & $\mathbf{50.22}$\,\dn{2.08} & $\mathbf{52.46}$\,\dn{4.77} & $\mathbf{90.14}$\,\dn{0.68} & $\mathbf{37.13}$\,\dn{1.08} & $\mathbf{52.08}$\,\dn{4.46} \\
% \bottomrule
% \end{tabular}
% }
% \caption{Results on the adversarial split of DRFA. Subscripts denote the absolute change relative to the orginal split (Table~\ref{tab:main_results}).}
% \label{tab:adv_results}
% \end{table*}
